MUSE: Multi-Knowledge Passing on the Edges, Boosting Knowledge Graph Completion

Knowledge Graph Completion (KGC) aims to predict the missing information in the (head entity)-[relation]-(tail entity) triplet. Deep Neural Networks have achieved significant progress in the relation prediction task. However, most existing KGC methods focus on single features (e.g., entity IDs) and sub-graph aggregation, which cannot fully explore all the features in the Knowledge Graph (KG), and neglect the external semantic knowledge injection. To address these problems, we propose MUSE, a knowledge-aware reasoning model to learn a tailored embedding space in three dimensions for missing relation prediction through a multi-knowledge representation learning mechanism. Our MUSE consists of three parallel components: 1) Prior Knowledge Learning for enhancing the triplets' semantic representation by fine-tuning BERT; 2) Context Message Passing for enhancing the context messages of KG; 3) Relational Path Aggregation for enhancing the path representation from the head entity to the tail entity. Our experimental results show that MUSE significantly outperforms other baselines on four public datasets, such as over 5.50% improvement in H@1 and 4.20% improvement in MRR on the NELL995 dataset. The code and all datasets will be released via https://github.com/NxxTGT/MUSE.

==> tables/Tab1.tex <==
\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}

==> tables/long-tail.tex <==
\begin{table}[!t]
\small
\centering
\resizebox{0.9\linewidth}{!}{
% \begin{table}
% \centering
% \caption{size=small,skip=5pt}
\label{tab:lt}
\begin{tabular}{l|l|c|c|c|c} 
\hline
\multirow{2}{*}{Scenarios}                     & \multirow{2}{*}{Methods} & FB15k-237              & WN18                   & WN18RR                                               & NELL995                 \\ 
\cline{3-6}
                                               &                          & H@1                    & H@1                    & H@1                                                  & H@1                     \\ 
\hline
\multirow{2}{*}{Limited Information Set (LIS)} & PathCon                  & 0.917                  & 0.983                  & 0.878                                                & 0.719                   \\
                                               & \textbf{MUSE}            & \textbf{0.975~}        & \textbf{0.992}         & \textbf{0.948}                                       & \textbf{0.858}          \\ 
\hline
\multirow{2}{*}{Rich Information Set (RIS)}    & PathCon                  & 0.962                  & 0.983                  & 0.967                                                & 0.897                   \\
                                               & \textbf{MUSE}            & \textbf{0.977}\uline{} & \textbf{0.991}\uline{} & \textcolor[rgb]{0.2,0.2,0.2}{\textbf{0.978}}\uline{} & \textbf{0.922}\uline{}  \\
\hline
\end{tabular}
}
\captionsetup{size=small,skip=5pt}
\caption{Relation Prediction in LIS and RIS.}
\label{tab:lt}
\vspace{-4mm}
\end{table}

==> tables/notation.tex <==
\begin{table}
% \resizebox{\linewidth}{!}{
\centering
\begin{tabular}{c|c}
\hline \text { Symbol } & \text { Description } \\
\hline ${h$, ${t}$ & \text { Head entity and tail entity } \\
r & \text { Relation type } \\
S_{e}^{i} & \text { Hidden state of edge } e \text { at iteration } i \\
M_{v}^{i} & \text { Message of node } v \text { at iteration } i \\
\mathcal{N}(e) & \text { Endpoint nodes of edge } e \\
\mathcal{N}(v) & \text { Neighbor edges of node } v \\
S_{(h, t)} & \text { Context representation of the entity pair }(h, t) \\
S_{h \rightarrow t} & \text { Path representation of all paths from } h \text { to } t \\
\alpha_{P} & \text { Attention weight of path } P \\
\mathcal{P}_{h \rightarrow t} & \text { Set of paths from } h \text { to } t \\
\hline
\end{tabular}
% }
\caption{Notation Used in This Paper.}
\label{tab:notation}
\end{table}


==> tables/settings.tex <==
\begin{table}[t]
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{l|c|c|c|c} 
\hline
Datasets       & FB15k-237 & WN18   & WN18RR & NELL995  \\ 
\hline
Layers        & 2         & 3      & 3      & 2        \\
Max Length    & 3         & 3      & 4      & 3        \\
Hiddens       & 64        & 64     & 64     & 64       \\
Learning Rate & 0.0001    & 0.0001 & 0.0005 & 0.0001   \\
\hline
\end{tabular}
}
\caption{The Settings in Our Experiment.}
\label{tab:1}
\end{table}
